Computing (or not) Quasi-Periodicity Functions of Tilings

We know that tilesets that can tile the plane always admit a quasi-periodic tiling [4, 8], yet they hold many uncomputable properties [3, 11, 21, 25]. The quasi-periodicity function is one way to measure the regularity of a quasi-periodic tiling. We prove that the tilings by a tileset that admits only quasi-periodic tilings have a recursively (and uniformly) bounded quasi-periodicity function. This corrects an error from [6, theorem 9] which stated the contrary. Instead we construct a tileset for which any quasi-periodic tiling has a quasi-periodicity function that cannot be recursively bounded. We provide such a construction for 1-dimensional effective subshifts and obtain as a corollary the result for tilings of the plane via recent links between these objects [1, 10].

==> dessins/macros.tex <==
% Commandes

\newcommand\sft[1]{\mathbf{#1}}
\newcommand\sshift[1]{\ensuremath{\mathbf{#1}}}
\newcommand\setofconf[1]{\ensuremath{\mathbf{#1}}}
\newcommand\groupe[1]{\ensuremath{\mathbf{#1}}}
\newcommand\grp{\ensuremath{\groupe{\mathcal{G}}}}
\newcommand\plan[1][\groupe{\Z^2}]{\ensuremath{\mathbf{#1}}}
\newcommand\plangrp{\plan[\grp]}
\newcommand\gengrp{\ensuremath{\mathbb{G}}}
\newcommand\couleur[1]{\mathbf{#1}}
\newcommand\motif[1]{\ensuremath{\mathbf{#1}}}
\newcommand\Distrib{\ensuremath{\left\{0,1\right\}^{\plan}}}
\newcommand\ensdef[1]{\ensuremath{\mathbf{#1}}}
\newcommand\domain[1]{\ensuremath{\mathcal{D}_{#1}}}
\newcommand\ens[1]{\mathbf{#1}}
\newcommand\enspav{\mathbf{T}}
\newcommand\dist[1]{\ensuremath{d_{#1}}}
\newcommand\distance[3]{\ensuremath{\dist{#1}(#2,#3)}}
\newcommand\norme[2]{\ensuremath{||#2||_{#1}}}
\newcommand\ouvert[1]{\ensuremath{\mathcal{#1}}}
\newcommand\open[1]{\ensuremath{\ouvert{O_{\motif{#1}}}}}
\newcommand\espace[1][\plan]{\ensuremath{\couleur{Q}^{#1}}}
\newcommand\repart{\ensuremath{\left\{0,1\right\}^{\plan}}}
\newcommand\espacegrp{\ensuremath{\couleur{Q}^{\plangrp}}}
\newcommand\ssmotif{\ensuremath{\sqsubseteq}}
\newcommand\extstrict{\ensuremath{\ll}}
\newcommand\conf[1]{#1}
\newcommand\morph[1]{#1}
\newcommand\orbite[2][\mathcal{G}]{\ensuremath{O_{\groupe{#1}}(\conf{#2})}}
\newcommand\egalmodshift{\ensuremath{=_{/\sigma}}}
\newcommand\shiftalone[1]{\ensuremath{\sigma_{#1}}}
\newcommand\shift[2]{\ensuremath{\shiftalone{#1}(\conf{#2})}}
\newcommand\class[1]{\ensuremath{\left<#1\right>}}
\newcommand\ForbPat{\ensuremath{\mathcal{F}}}
\newcommand\Tilings[1][\ForbPat]{\ensuremath{\enspav_{#1}}}
\newcommand\proj[1][f]{\ensuremath{\pi_{\morph{#1}}}}
\newcommand\rk{\ensuremath{\rho}}
\newcommand\engendre[1]{\ensuremath{\Gamma\left(\conf{#1}\right)}}
\newcommand\funper[1]{\ensuremath{\mathcal{F}_{\conf{#1}}}}
\newcommand\ensper[1]{\ensuremath{\mathcal{P}_{\conf{#1}}}}
\newcommand\gen[1]{#1}
\newcommand\rel[1]{#1}
\newcommand\pres[2]{\ensuremath{\left<\gen{#1}\mid\rel{#2}\right>}}
\newcommand\depl[1]{\ensuremath{\mathcal{S}_{#1}}}
\newcommand\lang[1]{\ensuremath{\mathcal{L}_{#1}}}
\newcommand\theorie[1]{\ensuremath{\mathcal{T}_{#1}}}
\newcommand\theorieinf[1]{\ensuremath{\theorie{#1}^{\infty}}}
\newcommand\neutre{e}
\newcommand\struct[1]{\ensuremath{\mathcal{#1}}}
\newcommand\interp[2]{\ensuremath{#1^{\struct{#2}}}}
\newcommand\pred[1]{\ensuremath{P_{#1}}}
\newcommand\formulemotif[1]{\ensuremath{\varphi_{\motif{#1}}}}
\newcommand\Lang[1]{\ensuremath{\mathcal{L}(#1)}}
\newcommand\vdistance[1]{#1}
\newcommand\boule[3]{\ensuremath{\mathcal{B}_{#1}(#2,\vdistance{#3})}}
\newcommand\cardcont{\ensuremath{2^{\aleph_0}}}
\newcommand\epsi{\varepsilon}
\newcommand\arbre[1]{#1}
\newcommand\langa{\ensuremath{\lang{\plan,\couleur{Q}}}}
\newcommand\theoriea{\ensuremath{\theorie{\plan,\couleur{Q},\ForbPat}}}
\newcommand\theorieainf{\ensuremath{\theorieinf{\plan,\couleur{Q},\ForbPat}}}
\newcommand\subst[1]{\ensuremath{#1}}

\newcommand\compl[1]{\ensuremath{#1^C}}
\newcommand\extsurpav[1]{\ensuremath{\ensdef{\mathcal{C}_{#1}}}}
\newcommand\domcritiquepavfini[1]{\ensuremath{\ensdef{\mathcal{X}_{#1}}}}

\newcommand\netiter[1]{\ensuremath{\conf{#1}^{\alpha,\beta}}}
\newcommand\netitersuite[1]{\ensuremath{(\netiter{#1}_n)_{n\in\N}}}
\newcommand\ilot[3]{\ensuremath{\mathcal{I}_{#1,#2}(\conf{#3})}}
\newcommand\efface[2]{\ensuremath{\mathcal{E}_{#1,#2}}}

\newcommand\La{\ensuremath{\mathcal{L}}}

\newcommand\cellcouleur[1]{\tikz[scale=.2]{\filldraw[fill=#1] (0,0) rectangle +(1,1);}}
\newcommand\latin[1]{\emph{#1}}
\newcommand\anglais[1]{\emph{#1}}
\newcommand\allemand[1]{\emph{#1}}
\newcommand\ie{\latin{i.e.}, }
\newcommand\eg{\latin{e.g.}, }
\newcommand\Z{\ensuremath{\mathbb{Z}}}
\newcommand\N{\ensuremath{\mathbb{N}}}

\newcommand\confsp[3]{\ensuremath{\conf{#1}_{\struct{#2},#3}}}
%% Inclusion des dessins
\newcommand\includetikz[1]{\opt{dessinetikz}{\input #1}\opt{pdftikz}{\includegraphics{#1.pdf}}}
\newcommand\includempost[2]{\opt{dessinempost}{\includegraphics[#1]{metapost/#2}}}
\newcommand\unif[1]{\ensuremath{\overline{#1}}}
\newcommand\bandeinf[1]{\ensuremath{\motif{#1}^{\updownarrow\omega}}}


\newcommand\qpfunc[1]{\ensuremath{\mathcal{Q}_{#1}}}
\newcommand\qppat[2]{\ensuremath{n_{(\motif{#1},#2)}}}
\newcommand\qppatloc[2]{\ensuremath{m_{(\motif{#1},#2)}}}
\newcommand\fourpat[3]{
\ensuremath{\motif{#1}_{|[-#2-#3;-#2]^2}},
\ensuremath{\motif{#1}_{|[-#2-#3;-#2]\times[#2;#2+#3]}},
\ensuremath{\motif{#1}_{|[#2;#2+#3]\times[-#2-#3;-#2]}},
\ensuremath{\motif{#1}_{|[#2;#2+#3]^2}}}


\newcommand\mgreen{green!75!black!50}
\newcommand\mmgreen{green!37!black!25}
\newcommand\mblue{blue!100!black!20}
\newcommand\mlblue{blue!70!black!50}
\newcommand\mmblue{blue!50!black!10}

